GDPO: Group reward-Decoupled Normalization Policy Optimization for Multi-reward RL Optimization

As language models become increasingly capable, users expect them to provide not only accurate responses but also behaviors aligned with diverse human preferences across a variety of scenarios. To achieve this, Reinforcement learning (RL) pipelines have begun incorporating multiple rewards, each capturing a distinct preference, to guide models toward these desired behaviors. However, recent work has defaulted to apply Group Relative Policy Optimization (GRPO) under multi-reward setting without examining its suitability. In this paper, we demonstrate that directly applying GRPO to normalize distinct rollout reward combinations causes them to collapse into identical advantage values, reducing the resolution of the training signal and resulting in suboptimal convergence and, in some cases, early training failure. We then introduce Group reward-Decoupled Normalization Policy Optimization (GDPO), a new policy optimization method to resolve these issues by decoupling the normalization of individual rewards, more faithfully preserving their relative differences and enabling more accurate multi-reward optimization, along with substantially improved training stability. We compare GDPO with GRPO across three tasks: tool calling, math reasoning, and coding reasoning, evaluating both correctness metrics (accuracy, bug ratio) and constraint adherence metrics (format, length). Across all settings, GDPO consistently outperforms GRPO, demonstrating its effectiveness and generalizability for multi-reward reinforcement learning optimization.

==> sections/preliminary.tex <==
% \xin{this section is primarily paraphrasing GRPO equations in the multi-objective cases. Let's merge this section into Sec 3.}

Recent advancements such as Group Relative Policy Optimization (GRPO)~\citep{guo2025deepseek} and its variants, including DAPO~\citep{yu2025dapo} and Reinforce++-Baseline~\citep{hu2025reinforce++}, have emerged as widely adopted reinforcement learning algorithms due to their efficiency and simplicity. 
In contrast to Proximal Policy Optimization (PPO)~\cite{schulman2017proximal}, GRPO eliminates the need for a value model by leveraging group-relative advantage estimation for policy updates.

Currently, GRPO has been primarily employed for optimizing a single-objective reward, typically focusing on accuracy. 
However, as model capability continues to grow, recent works have increasingly sought to optimize multiple rewards, such as response length constraint and formatting quality, in addition to accuracy~\citep{liu2025laser,qian2025toolrl,aggarwal2025l1}, to better align with human preferences. Existing approaches for multi-reward RL generally adopt a straightforward strategy: summing all reward components and applying GRPO directly.

Formally, for a given question–answer pair $(q_i, o_j)$, where the behavior policy $\pi_{\theta_{\mathrm{old}}}$ samples a group of $G$ responses $\{o_j\}_{j=1}^G$, and assuming $n$ objectives, the aggregated reward for the $j$-th response is computed as the sum of each objective’s reward:
\begin{equation}
r^{(i,j)}_{\text{sum}} = r_1^{(i,j)} + \cdots + r_n^{(i,j)}
\label{eq:grpo_sum}
\end{equation}
The group-relative advantage for the $j$-th response is then obtained by normalizing the group-level aggregated rewards:
\begin{equation}
A^{(i,j)}_{\text{sum}} =
\frac{
r_{\text{sum}}^{(i,j)} - \mathrm{mean}\{ r_{\text{sum}}^{(i,1)}, \ldots, r_{\text{sum}}^{(i,G)}\}
}{
\mathrm{std}\{ r_{\text{sum}}^{(i,1)}, \ldots, r_{\text{sum}}^{(i,G)} \}
}
\label{eq:grpo_advantage}
\end{equation}
The corresponding multi-reward GRPO optimization objective can then be expressed as:

\begin{equation}
\mathcal{J}_{\mathrm{GRPO}}(\theta) = 
\mathbb{E}_{(q_i,o_j) \sim D,\; \{o_j\}_{j=1}^G \sim \pi_{\theta_{\mathrm{old}}}(\cdot|q)} 
\left[
\frac{1}{G} \sum_{j=1}^{G} \frac{1}{|o_j|} \sum_{t=1}^{|o_j|}
\min \left(
s_{i,t}(\theta)\, A^{(i,j)}_{\text{sum}},\;
\mathrm{clip}(s_{i,t}(\theta), 1 - \epsilon, 1 + \epsilon)\,A^{(i,j)}_{\text{sum}}
\right)
\right]
\label{eq:grpo}
\end{equation}
where $s_t(\theta) = \frac{\pi_{\theta}(o_j^t \,|\, q, o_j^{<t})}{\pi_{\theta_{\mathrm{old}}}(o_j^t \,|\, q, o_j^{<t})}$ 
and $\epsilon$ denotes the clipping threshold. For clarity, we omit the KL-divergence loss term in this formulation. 


% Following~\citep{}, we adopt the token-level loss normalization from DAPO across all experiments. 
% \mathcal{J}_{\mathrm{GRPO}}(\theta) = 
% \mathbb{E}_{(q_i,o_j) \sim D,\; \{o_j\}_{j=1}^G \sim \pi_{\theta_{\mathrm{old}}}(\cdot|q)} 
% \left[
% \frac{1}{\sum_{j=1}^G |o_j|} 
% \sum_{j=1}^G \sum_{t=1}^{|o_j|}
% \min \left(
% s_{i,t}(\theta)\, A^{(i,j)}_{\text{sum}},\;
% \mathrm{clip}(s_{i,t}(\theta), 1 - \epsilon, 1 + \epsilon)\,A^{(i,j)}_{\text{sum}}
% \right)
% \right]
